RADAR: Robust AI-Text Detection via Adversarial Learning

Recent advances in large language models (LLMs) and the intensifying popularity of ChatGPT-like applications have blurred the boundary of high-quality text generation between humans and machines. However, in addition to the anticipated revolutionary changes to our technology and society, the difficulty of distinguishing LLM-generated texts (AI-text) from human-generated texts poses new challenges of misuse and fairness, such as fake content generation, plagiarism, and false accusations of innocent writers. While existing works show that current AI-text detectors are not robust to LLM-based paraphrasing, this paper aims to bridge this gap by proposing a new framework called RADAR, which jointly trains a robust AI-text detector via adversarial learning. RADAR is based on adversarial training of a paraphraser and a detector. The paraphraser's goal is to generate realistic content to evade AI-text detection. RADAR uses the feedback from the detector to update the paraphraser, and vice versa. Evaluated with 8 different LLMs (Pythia, Dolly 2.0, Palmyra, Camel, GPT-J, Dolly 1.0, LLaMA, and Vicuna) across 4 datasets, experimental results show that RADAR significantly outperforms existing AI-text detection methods, especially when paraphrasing is in place. We also identify the strong transferability of RADAR from instruction-tuned LLMs to other LLMs, and evaluate the improved capability of RADAR via GPT-3.5-Turbo.

==> figures/iBLEU.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/iBLEU.png}
    \caption{ Evaluation of RADAR's paraphraser versus its initial version (T5-large) on Quora Question Pairs.
    \label{fig:iBLEU} 
    } 
\vspace{-4mm}
\end{figure}

==> figures/model_size.tex <==
\begin{figure}[htb]
\vspace{-2mm}
    \centering
    \begin{subfigure}[t]{0.49\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/model_size_wo.png}
        \caption{w/o paraphraser \label{fig:model_size_wo}}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/model_size_unseen.png}
        \caption{unseen paraphraser \label{fig:model_size_unseen}}
    \end{subfigure}
    \caption{Ablation study on model size. The experiments are conducted with GPT-2-XL (target LLM). The result is the average AUROC score of the 4 datasets. \PYB{Add ``Detector model size'' to the legend }\XMB{Already in the top of the figure}
    \label{fig:model_size}}
\end{figure}

==> figures/paraphrase_on_different_side.tex <==
\begin{figure}[htb]
    \centering
    \begin{subfigure}[t]{0.49\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/model_side_attack.png}
        \caption{Paraphrase AI-text. \label{fig:model_side_attack}}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/human_side_attack.png}
        \caption{Paraphrase Human-text. \label{fig:human_side_attack}}
    \end{subfigure}
    \caption{Paraphrase on both sides. \PYB{Not a very good diagram}
    \label{fig:paraphrase_side}}
\end{figure}

==> pesudo_code/ppo.tex <==

\begin{algorithm}
\caption{Generator Training Process}\label{alg:cap}
\begin{algorithmic}
\Require $n \geq 0$
\Ensure $y = x^n$
\State $y \gets 1$
\State $X \gets x$
\State $N \gets n$
\While{$N \neq 0$}
\If{$N$ is even}
    \State $X \gets X \times X$
    \State $N \gets \frac{N}{2}$  \Comment{This is a comment}
\ElsIf{$N$ is odd}
    \State $y \gets y \times X$
    \State $N \gets N - 1$
\EndIf
\EndWhile
\end{algorithmic}
\end{algorithm}


==> tables/compare_schemas.tex <==
\begin{table}
    \centering
    \small
    \caption{AUROC score averaged over 8 target LLMs. RADAR-Seen Paraphraser means the paraphraser used in RADAR~($\mathcal{G}_\sigma$). RADAR-Unseen Paraphraser is OpenAI's GPT-3.5-Turbo API.~The notations \{\wofirst,\seenfirst,\unseenfirst\}/    \{\wosecond,\seensecond,\unseensecond\}  denote the best/second-best method of \{\textcolor{green}{w/o},\textcolor{blue}{RADAR-Seen},\textcolor{red}{RADAR-Unseen}\} paraphraser setting for each dataset. }
    \resizebox{\linewidth}{!}{
     \begin{tabular}{c|c|c|c|c|c|c} 
    \hline
    \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Evaluation Schema}}   & \multicolumn{4}{c}{\textbf{Evaluation Dataset}}  \\
    \cline{3-7}
                                    &                                           & \textbf{Xsum}   & \textbf{SQuAD}  & \textbf{WP} & \textbf{TOFEL} & \textbf{Average}\\ 
    \hline
    \multirow{3}{*}{log p}           & {\color{green}w/o Paraphraser}                                              & 0.882   & 0.868         & 0.967\wosecond        & 0.832 &0.887 \\ 
                                    & {\color{blue}RADAR-Seen Paraphraser}                                            
    & 0.230	& 0.156	& 0.275	& 0.130 &0.198\\
                                    & {\color{red}RADAR-Unseen Paraphraser}                                            
    & 0.266	& 0.343	& 0.641	& 0.438  &0.422       \\
    \hline
    \multirow{3}{*}{rank}           & {\color{green}w/o Paraphraser}                                              &  0.722	& 0.752	 & 0.814	 & 0.731 &0.755\\
                                    & {\color{blue}RADAR-Seen Paraphraser}                                            
    & 0.334	& 0.282	& 0.357	& 0.163 &0.284\\
                                    & {\color{red}RADAR-Unseen Paraphraser}                                            
    & 0.433	&0.436	&0.632	&0.342   &0.461     \\
    \hline
    \multirow{3}{*}{log rank}        & {\color{green}w/o Paraphraser}                                                & 
 0.902         & 0.893\wosecond        & 0.975\wofirst  & 0.847\wosecond &0.904\wofirst\\
                                    & {\color{blue}RADAR-Seen Paraphraser}                                            
    & 0.245	& 0.175	& 0.281	& 0.134 & 0.209\\
                                    & {\color{red}RADAR-Unseen Paraphraser}                                            
    & 0.282	& 0.371	& 0.632	& 0.421 &0.426
        \\
    \hline
    \multirow{3}{*}{entropy}        & {\color{green}w/o Paraphraser}                                              & 0.536	& 0.521	& 0.296	& 0.534 & 0.472
 \\
                                    & {\color{blue}RADAR-Seen Paraphraser}                                            
    & 0.796	& 0.845\seensecond	& 0.763	& 0.876\seensecond &0.820\seensecond\\
                                    & {\color{red}RADAR-Unseen Paraphraser}                                            
    & 0.779	&0.710\unseensecond	& 0.499	& 0.618 &0.651\unseensecond
        \\
    \hline
    \multirow{3}{*}{DetectGPT}        & {\color{green}w/o Paraphraser}                                              & 0.874	& 0.790	& 0.883	& 0.919\wofirst &0.867
 \\
                                    & {\color{blue}RADAR-Seen Paraphraser}                                            
    & 0.191	& 0.105	& 0.117	& 0.177 &0.159\\
                                    & {\color{red}RADAR-Unseen Paraphraser}                                            
    & 0.360	& 0.384	& 0.609	& 0.630\unseensecond & 0.434
        \\
    \hline
    \multirow{3}{*}{RoBERTa-based Detector}        & {\color{green}w/o Paraphraser}                                              & 0.953\wofirst	& 0.914\wofirst	& 0.924	& 0.810 & 0.900\wosecond

 \\
                                    & {\color{blue}RADAR-Seen Paraphraser}                                            
    & 0.821\seensecond	& 0.842	& 0.892\seensecond	& 0.670 &0.806
 \\
                                    & {\color{red}RADAR-Unseen Paraphraser}                                            
    & 0.789\unseensecond	& 0.629	& 0.726\unseensecond	& 0.364 & 0.627

        \\
    \hline
    \multirow{3}{*}{RADAR}        & {\color{green}w/o Paraphraser}                                              & 0.934\wosecond	& 0.825	& 0.847\	& 0.820 &0.856
 \\
                                    & {\color{blue}RADAR-Seen Paraphraser}                                            
    & 0.920\seenfirst	& 0.927\seenfirst	& 0.908\seenfirst	& 0.932\seenfirst &0.922\seenfirst\\
                                    & {\color{red}RADAR-Unseen Paraphraser}                                            
    & 0.955\unseenfirst	& 0.861\unseenfirst	& 0.851\unseenfirst	& 0.763\unseenfirst & 0.857\unseenfirst
        \\
    \hline
    \end{tabular}  }
    \label{tab:conpare_scenarios}
\vspace{-4mm}
\end{table}

==> tables/main_results.tex <==
\begin{table*}[t]
    \centering
    \small
    % \resizebox{\linewidth}{!}{
     \begin{tabular}{l|l|l|l|l|l|l|l|l} 
    % \hline
    \hline
    \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{3B}} & \multicolumn{2}{c}{\textbf{5B}} & \multicolumn{2}{c}{\textbf{6B}} & \multicolumn{2}{c}{\textbf{7B}}\\
    \cline{2-9}
                                    & \textbf{Pythia} & \textbf{Dolly-v2}    & \textbf{Palmyra}    & \textbf{Camel}    & \textbf{GPT-J} & \textbf{Dolly-V1}   &  \textbf{Llama} &  \textbf{Vicuna}\\
    \hline
    \multicolumn{9}{l}{\textbf{White-Box detection}} \\
    \hline
    LogProbability                  & 0.822
                                    & 0.987
                                    & 0.887
                                    & 0.999
                                    & 0.812               
                                    & 0.931
                                    & 0.692
                                    & 0.969\\

    Rank                            & 0.777
                                    & 0.819
                                    & 0.779
                                    & 0.765
                                    & 0.771               
                                    & 0.785
                                    & 0.663
                                    & 0.678\\

    LogRank                         & 0.861
                                    & 0.985
                                    & 0.914
                                    & 0.998
                                    & 0.847               
                                    & 0.938
                                    & 0.734
                                    & 0.958\\
    Entropy                         & 0.552
                                    & 0.452
                                    & 0.495
                                    & 0.339
                                    & 0.533               
                                    & 0.470
                                    & 0.596
                                    & 0.338\\

    DetectGPT                       & 0.842
                                    & 0.988
                                    & 0.899
                                    & 0.973
                                    & 0.799               
                                    & 0.821
                                    & 0.705
                                    & 0.906\\
    \hline
    \multicolumn{9}{l}{\textbf{Black-Box detection}} \\
    \hline
    RoBERTa-based Detector          & 0.959
                                    & 0.874
                                    & 0.969
                                    & 0.859
                                    & 0.934               
                                    & 0.933
                                    & 0.837
                                    & 0.839\\
    RADAR                           & 0.854
                                    & 0.769
                                    & 0.916
                                    & 0.920
                                    & 0.820               
                                    & 0.859
                                    & 0.808
                                    & 0.906\\
    \hline
    % \hline
    \end{tabular} 
    \caption{AUROC for detecting samples from the given model on the given dataset for DetectGPT and four previously proposed criteria
(500 samples used for evaluation). From 1.5B parameter GPT-2 to 20B parameter GPT-NeoX, DetectGPT consistently provides the most
accurate detections. Bold shows the best AUROC within each column (model-dataset combination); asterisk (*) denotes the second-best
AUROC. Values in the final row show DetectGPT’s AUROC over the strongest baseline method in that column.}
    \label{tab:main_results}
\end{table*}
